Interpolation Learning With Minimum Description Length

We prove that the Minimum Description Length learning rule exhibits tempered overfitting. We obtain tempered agnostic finite sample learning guarantees and characterize the asymptotic behavior in the presence of random label noise.

==> colt_includes.tex <==
\usepackage[most]{tcolorbox}
\definecolor{ForestGreen}{RGB}{34, 139, 34}
\newcommand{\greenbox}[1]{
    \vspace{0.15cm}
    { \small
    \begin{tcolorbox}[enhanced, colback=ForestGreen!12, parbox=false]
    #1
    \end{tcolorbox}
    }
}
% \usepackage{todonotes}
\newcommand{\nnote}[1]{ \begin{footnotesize}$\ll$\textsf{\color{blue} Naren: { #1}}$\gg$\end{footnotesize}}
\newcommand{\natinote}[1]{ \begin{footnotesize}$\ll$\textsf{\color{magenta} Nati: { #1}}$\gg$\end{footnotesize} }
\newcommand{\removed}[1]{}
\newcommand{\natinotelater}[1]{}
% \newcommand{\natinote}[1]{\ifnotes \begin{footnotesize}$\ll$\textsf{\color{magenta} Nati: { #1}}$\gg$\end{footnotesize} \fi}

%%%%%%%%%%%%%%%%%%%%%%%%% Enclosures
\newcommand{\inparen}[1]{\left(#1\right)}             %\inparen{x+y}  is (x+y)
\newcommand{\inbraces}[1]{\left\{#1\right\}}           %\inbrace{x+y}  is {x+y}
\newcommand{\insquare}[1]{\left[#1\right]}             %\insquare{x+y}  is [x+y]
\newcommand{\inangle}[1]{\left\langle#1\right\rangle} %\inangle{A}    is <A>
\newcommand{\inmod}[1]{\inparen{\mathrm{mod}\ #1}}
\newcommand{\B}{\inbraces{0,1}}
\newcommand{\pmone}{\inbraces{\pm1}}
\newcommand{\indicator}[1]{\mathbbm{1}\!\inbraces{#1}}
\newcommand{\abs}[1]{\ensuremath{\left\lvert #1 \right\rvert}}
\newcommand{\norm}[1]{\ensuremath{\left\lVert #1 \right\rVert}}
\newcommand{\opnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\mathrm{op}}}}
\newcommand{\maxnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\infty}}}
\newcommand{\fnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{F}}}
\newcommand{\lipnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{\mathrm{Lip}}}}
\newcommand{\onenorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{1}}}
\newcommand{\zeronorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{0}}}
\newcommand{\nuclearnorm}[1]{\ensuremath{\left\lVert #1 \right\rVert_{*}}}
\newcommand{\smallnorm}[1]{\ensuremath{\lVert #1 \rVert}}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\mydot}[2]{\ensuremath{\left\langle #1, #2 \right\rangle}}
\newcommand{\mysmalldot}[2]{\ensuremath{\langle #1, #2 \rangle}}
\newcommand{\ip}[1]{\left\langle #1 \right\rangle}
\newcommand{\myfunc}[3]{#1\colon#2\to#3}

% Character Shortcuts
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%%%%%%%%%% Symbols and Fonts
\def\from{:}
\def\to{\rightarrow}
\def\eps{\varepsilon}
% \def\epsilon{\varepsilon}
\def\e{\varepsilon}
\def\eps{\varepsilon}
\def\d{\delta}
% \def\phi{\varphi}
\def\cal{\mathcal}
\def\xor{\oplus}
\def\ra{\rightarrow}
\def\implies{\Rightarrow}
\def\psdgeq{\succeq} 
\renewcommand{\bar}{\overline} 
\newcommand{\ol}{\overline}

%% Operators

\newcommand{\E}{\mathbb{E}}
\renewcommand{\Pr}{\mathsf{Pr}}
\newcommand{\exv}[1]{\E\insquare{#1}}
\newcommand{\exvv}[2]{\underset{#1}{\E}\insquare{#2}}
\newcommand{\expv}[1]{\mathsf{exp}\inparen{#1}}
\newcommand{\prv}[1]{\Pr\insquare{#1}}
\newcommand{\prvv}[2]{\underset{#1}{\Pr}\insquare{#2}}
\newcommand{\logv}[1]{\log\inparen{#1}}
\newcommand{\diag}[1]{\mathsf{diag}\inparen{#1}}
\newcommand{\diam}[1]{\mathsf{diam}\inparen{#1}}
\newcommand{\linf}{\ell_{\infty}}
\newcommand{\costv}[1]{\cost\inparen{#1}}
\newcommand{\err}[2]{\mathsf{err}_{#1}\inparen{#2}}
\newcommand{\signv}[1]{\sign\inparen{#1}}
\newcommand{\trv}[1]{\Tr\inparen{#1}}

% For algorithms
\usepackage{algorithm}
\usepackage{algorithmic}

% extra environments
\newtheorem{fact}[theorem]{Fact}


%%%%%%%%%%%% Fractions
% commands for fractions 
\usepackage{nicefrac}
% poor man's fraction
\newcommand{\flatfrac}[2]{#1/#2}
\newcommand{\varflatfrac}[2]{#1\textfractionsolidus#2}
\let\nfrac=\nicefrac
\let\ffrac=\flatfrac

% fonts
\usepackage{bbm}

\usepackage{wrapfig}


==> scratch.tex <==
\nnote{some warmup about the taxonomy of overfitting and a teaser about what we study, \cite{taxonomy}}

\subsection{Learning Problem Setup}

The learner is given a \textit{training set} $S = \inbraces{(x_1, y_1), \dots, (x_n, y_n)}$, where each $(x_i, y_i)$ is independently and identically distributed according to some (possibly unknown) distribution $\cD$. The learner's task is to choose $n$ and apply a \textit{learning rule} over known some set of functions $\cH$ to obtain a function $\hhat \in \cH$. We say the \textit{generalization error} of a function $h$ is at most $\eps$ if $L_{\cD}(h) \coloneqq \prvv{(x,y) \sim \cD}{\hhat(x) \neq y} \le \eps$. We assess the quality of the learner's solution $\hhat$ by comparing the generalization error of $\hhat$ against the (limit of) the generalization error of the best solution in $\cH$, i.e., $\underset{h \in \cH}{\inf} L_{\cD}(h)$. Broadly, the goal of the learner's learning rule is to obtain a function $\hhat$ satisfying $\exvv{S \sim \cD^n}{L_{\cD}(\hhat)} \le \underset{h \in \cH}{\inf} L_{\cD}(h) + \eps$, where $\eps$ may depend on $n$.

On top of this, we consider several noise models. We say we are in the \textit{realizable} setting if there exists a function $\hstar \in \cH$ such that for all $(x,y)\sim\cD$ we have $y = \hstar(x)$. We say we are in the \textit{random classification noise} setting if there exists a function $\hstar \in \cH$ such that for all $(x,y)\sim\cD$ we have $y = \hstar(x) \oplus z$ where $z$ is a Bernoulli-$\alpha$ random variable independent of $x$ and $a \oplus b$ is the $\F_2$ addition of two bits $a,b$. Otherwise, we are in the \textit{agnostic} case. 

We now introduce the learning rule we study in this paper. See Definition \ref{def:mdl}.
\begin{definition}[Minimum Description Length (MDL) learning rule]
\label{def:mdl}
The MDL hypothesis is the hypothesis with the shortest description length among all hypotheses that are consistent with the training data. Formally, given a training set $S$, the rule outputs the solution to the optimization problem
\begin{align*}
    \mathsf{MDL}(S) \coloneqq \underset{h(x) = y, \textnormal{ for all } (x,y) \in S}{\textnormal{argmin}} \abs{h}
\end{align*}
where $\abs{h}$ denotes the length of the shortest Turing machine that agrees with $h$ on all possible inputs $x$.
\end{definition}

It is well-known (see, e.g., \nnote{cite}) that in the realizable case, the MDL learning rule enjoys the generalization guarantee in Fact \ref{fact:mdl_generalization}.

\begin{fact}
\label{fact:mdl_generalization}
In the realizable setting, if $S$ consists of $n$ independent and identically distributed samples from $\cD$, then with probability $1-\delta$ over the draw of $S$, the MDL learning rule satisfies
\begin{align*}
    L_{\cD}(\mathsf{MDL}(S)) \le \frac{\abs{\mathsf{MDL}(S)} + \logv{\nfrac{2}{\delta}}}{2n}
\end{align*}
\nnote{citation? i copied this out of the lecture notes}
\end{fact}

\subsection{Contributions and Discussion}

Our main result is Theorem \ref{thm:finite_sample_mdl_rcn}.

\begin{theorem}
\label{thm:finite_sample_mdl_rcn}
Let $\cD$ be such that for $(x,y) \sim \cD$, we have $x \sim \unif[0,1]$. Let $S$ consist of $n$ independent and identical draws from $\cD$. If we are in the random classification noise setting for some base classifier $\hstar$, then we have
\begin{align*}
    \abs{\mathsf{MDL}(S)} &\le \abs{\hstar} + nH(\alpha) + o(n)
\end{align*}
where $H(\alpha)$ is the binary entropy function, i.e., $H(\alpha) = -\alpha\log\alpha - (1-\alpha)\logv{1-\alpha}$. 
% This implies a generalization bound
% \begin{align*}
%     L_{\cD}\inparen{\mathsf{MDL}(S)} \le 2\alpha(1-\alpha) + \sqrt{H(\alpha) + o(1)}
% \end{align*}
\end{theorem}

\nnote{Informally, what are the main contributions?}
\nnote{What are the quantifiers? If these claims hold ``in expectation'', what is the expectation taken over?}
\begin{itemize}
    \item Tight finite-sample generalization guarantee for MDL learning rule where the data is $\unif[0,1]$ and the problem is well-specified with random classification noise.
    \item The above shows tempered overfitting for MDL in the well-specified setting with random classification noise.
    \item Guarantee for the agnostic case with random classification noise, but this is not necessarily tight.
\end{itemize}
% \nnote{Proof outline:}
% \begin{itemize}
%     \item If there exists a program of length $\sim n\cdot H(\alpha) + \abs{\hstar}$ that fits the training set perfectly, then its population error converges to $2\alpha(1-\alpha)$ in $n$ (in the random classification model).
%     \item When $\cD = \unif[0,1]$, there exists a program of length $\sim n \cdot H(\alpha)$ that fits the training set perfectly.
%     \item This is tight -- any program that fits the training set perfectly must have length at least $n \cdot H(\alpha) + \abs{\hstar}$.
% \end{itemize}

\subsection{Notation and Technical Overview}

In this subsection, we establish our notation. We then give a high level overview of our methods.

\subsubsection{Notation and Terminology}

\paragraph{General notation} In this paper, we work extensively with distributions and random variables. We denote random variables with uppercase letters unless otherwise specified. We express distributions in several ways. We let $\unif[0,1]$ denote the uniform distribution over the interval $[0,1]$. We let $\ber{\alpha}$ denote a Bernoulli random variable with $1$-probability $\alpha$. \nnote{RN derivatives}. If $\cD$ is a distribution, we denote the $n$-fold product distribution of $\cD$ as $\cD^n$. For $x, y \in \inbraces{0,1}$, we denote the $\F_2$ sum of $x$ and $y$ as $x \oplus y$. 

For a labeled set of examples $S$ consisting of $(x,y)$ pairs where $x$ is the example and $y$ is the label, we write $S_x$ to denote the set of all examples and $S_y$ to denote the set of all labels. For a specific $x$, if $x$ appears in $S_x$ exactly once, then we write $S[x]$ to denote the value of $y$ associated with $x$.

For a number $x$, we let $x[i]$ be the $i$th digit of its binary expansion.

\subsubsection{Existence of a Short Classifier}

Our proof of Theorem \ref{thm:finite_sample_mdl_rcn} involves a few parts. In the first part, we prove the existence of a program that fits $S$ that also has length at most $\abs{\hstar} + n\cdot H(\alpha) + o(n)$. For an overview of this, see Algorithm \ref{alg:main_program}.

\begin{algorithm}[H]
\caption{Constructing a short interpolating program on $S$\label{alg:main_program}}
\begin{algorithmic}[1]
    \STATE \textbf{Input}: Training set $S$ of size $n$.
    \STATE \textbf{Output}: Hypothesis $\hhat$ such that for all $(x,y) \in S$, $\hhat(x) = y$.
    \STATE Let $\cA$ be a program that, given $(x,y) \in S$, outputs $\indicator{y \neq \hstar(x)}$.
    \STATE \textbf{Output}: The program ``\texttt{return $\hstar(x) \oplus \cA(x)$}''
\end{algorithmic}
\end{algorithm}

It is easy to see that Algorithm \ref{alg:main_program} outputs a program that memorizes the training set. We now need to analyze the length of the program that Algorithm \ref{alg:main_program} outputs. To evaluate $\hstar(x) \oplus \cA(x)$, we can separately compute $\hstar(x)$ and $\cA(x)$ before combining them with the $\oplus$ operator. We can compute $\hstar(x)$ using a program of length $\abs{\hstar}$. 

It remains to identify a $\cA$ that is short with high probability over the draws of $S$. This is the main technical challenge we face in our constructive result. To illustrate this difficulty, we start with a strawman solution.  Let $S'$ consist of the pairs $(x,y)$ such that $y \neq \hstar(x)$. A natural candidate for $\cA$ that attains generalization error $\sim \alpha$ is the program that memorizes the examples $x$ belong to $S'$. Unfortunately, in this case, $\cA$ must write down exactly the examples $x \in S_x'$, which requires an infinite length description.

This reveals a constraint we face when building $\cA$. In general, we cannot afford to store very much information about the actual values of $x$, as this can rapidly increase the program length of $\cA$. \nnote{how to best word the main difficulty in the existence result?}

\subsubsection{Bounding Any Program Memorizing Noisy Labels}

\nnote{outline of how we get the tightness result}

% We build the tools to prove Theorem \ref{thm:short_hash_table} across two subsections. In Section \ref{subsec:short_hash_table_construct}, we give a procedure to construct and evaluate $\cA$. In Section \ref{subsec:short_hash_table_tight}, we show that our construction is tight, in the sense that any $\cA$ of length $n\cdot H(\alpha) + o(n)$ must have false-positive rate $\sim \alpha$.

% \subsection{Constructing $\cA$}
% \label{subsec:short_hash_table_construct}

% The main result of this subsection is Theorem \ref{thm:short_hash_table_existence}.

% \begin{theorem}
% \label{thm:short_hash_table_existence}
% The below holds with probability $\ge 1-\delta$ over the draw of $S$.

% There exists a program satisfying the requirements stated in Problem \ref{problem:short_hash_table}. This program takes $n\cdot H(\alpha) + o(n)$ bits to express.

% Furthermore, no program satisfying the properties stated in Problem \ref{problem:short_hash_table} can be stored in fewer than $n \cdot H(\alpha)$ bits.
% \end{theorem}

% \begin{proof}[Upper bound, Theorem \ref{thm:short_hash_table_existence}]
% Let the target program be $\cA$.

% We give two functions. The first function (Algorithm \ref{alg:construct_short_hash_table}) constructs $\cA$ and the second (Algorithm \ref{alg:evaluate_short_hash_table}) shows how to evaluate queries.
% \begin{algorithm}[H]
% \caption{Constructing $\cA$\label{alg:construct_short_hash_table}}
% \begin{algorithmic}[1]
%     \STATE \textbf{Input}: Failure probability parameter $\delta$; $S \sim \inparen{\unif[0,1], \ber{\alpha}}^n$
%     \STATE \textbf{Output}: Program $\myfunc{\cA}{\insquare{0,1}\times\N\times\R}{\B}$ and parameter $k$ such that for all $x \in S_x$, $\cA(x,k) = S[x]$ and $\prvv{x\sim\cD}{\cA(x) = 1}\le \alpha$.
%     \STATE Let $S_x = \inbraces{x_1,\dots,x_n}$.
%     \STATE Let $\alphahat$ be a truncation of $\alpha$ such that $\alphahat$ takes at most $b$ bits to store.
%     \STATE Let $z_i$ be a sequence of i.i.d $\alphahat$-biased random bits extracted from $x_i$, for all $i \in [n]$.
%     \STATE Let $k$ be the smallest integer such that $z_i[k] = S[x_i]$.
%     \STATE Given $k$, let Algorithm \ref{alg:evaluate_short_hash_table} be the function to evaluate $\cA(x)$.
%     \STATE \textbf{Output}: $\cA$ (i.e., Algorithm \ref{alg:evaluate_short_hash_table}), $k$, and $\alphahat$.
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{Evaluating $\cA$\label{alg:evaluate_short_hash_table}}
% \begin{algorithmic}[1]
%     \STATE \textbf{Input}: $x \sim \unif[0,1]$, seek-distance $k$, approximation to $\alpha$ (i.e., $\alphahat$).
%     \STATE \textbf{Output}: $\cA(x)$
%     \STATE Initialize index $j = 1$.
%     \FOR{$i = 1, \dots, k$}
%         \STATE Initialize seeker $s = 1$.
%         \WHILE{$x[j:j+s] = \alphahat[1:s]$ and $s \le \mathsf{Length}(\alphahat)$}
%             \STATE Update $s \gets s+1$
%         \ENDWHILE
%         \IF{$x[j:j+s] > \alphahat$ and $i = k$}
%             \STATE \textbf{Output}: $1$
%         \ENDIF
%         \IF{$x[j:j+s] < \alphahat$ and $i = k$}
%             \STATE \textbf{Output}: $0$
%         \ENDIF
%         \STATE Update $j \gets j+s$
%     \ENDFOR
%     \STATE \textbf{Output}: $1$
% \end{algorithmic}
% \end{algorithm}

% \nnote{Give the probability that an $\alpha$-biased sequence is not in a sufficient $\alphahat$-typical set}

% Notice that Algorithm \ref{alg:evaluate_short_hash_table} extracts $\alpha$-biased independent bits from its input $x$ and returns the $k$th bit. Thus, calling Algorithm \ref{alg:evaluate_short_hash_table} on every $x \in S$ returns the corresponding value of $y$.

% It remains to analyze the length of $\cA, k, \alphahat$. Observe that Algorithm \ref{alg:evaluate_short_hash_table} takes constant space to express, so it is enough to count the bit complexity of $k$ and $\alphahat$. We first prove Lemma \ref{lemma:k_small}. 

% \begin{lemma}
% \label{lemma:k_small}
% The value of $k$ output by Algorithm \ref{alg:construct_short_hash_table} takes at most
% \begin{align*}
%     \log\logv{\nfrac{1}{\delta}}+\abs{S}\inparen{\kld{\alpha}{\alphahat} + H(\alpha) + \frac{\alpha}{\alphahat}\cdot\sqrt{\frac{3}{\alpha\abs{S}}}\logv{\nfrac{2}{\delta}}}
% \end{align*}
% bits to represent with probability $1-2\delta$.
% \end{lemma}
% \begin{proof}[Proof of Lemma \ref{lemma:k_small}]
% Let $S'$ consist of all $(x,y)$ such that $S[x] = 1$.

% To bound $k$, observe that $k$ is a geometric random variable with success probability $(\alphahat)^{\abs{S'}}(1-\alphahat)^{\abs{S}-\abs{S'}}$. Thus, we have, for any $T$
% \begin{align*}
%     \prvv{z_i}{k \ge T} = \inparen{1-\alphahat^{\abs{S'}}(1-\alphahat)^{\abs{S}-\abs{S'}}}^{T} \le \expv{-T\alphahat^{\abs{S'}}(1-\alphahat)^{\abs{S}-\abs{S'}}}
% \end{align*}
% Choosing $T = \alphahat^{-\abs{S'}}(1-\alphahat)^{-\abs{S}+\abs{S'}}\cdot\logv{\nfrac{1}{\delta}}$ and plugging this into the above gives
% \begin{align*}
%     \prvv{z_i}{k \ge T} = \prvv{z_i}{k \ge \alphahat^{-\abs{S'}}(1-\alphahat)^{-\abs{S}+\abs{S'}}\cdot\logv{\nfrac{1}{\delta}}} \le \delta
% \end{align*}
% which means with probability $1-\delta$, $k$ takes at most
% \begin{align*}
%     \logv{k \ge \alphahat^{-\abs{S'}}(1-\alphahat)^{-\abs{S}+\abs{S'}}\cdot\logv{\nfrac{1}{\delta}}} = \log\logv{\nfrac{1}{\delta}}+\abs{S'}\logv{\frac{1}{\alphahat}} + \inparen{\abs{S}-\abs{S'}}\logv{\frac{1}{1-\alphahat}}
% \end{align*}
% bits to store. It remains to bound $\abs{S'}$ up to probability $1-\delta$. Using a Chernoff bound, we have
% \begin{align*}
%     \prvv{\abs{S'} \subset_{\alpha} \abs{S}}{\abs{S'} \in \insquare{1\pm\eta}\alpha\abs{S}} \ge 1-2\expv{-\nfrac{\eta^2\alpha\abs{S}}{3}}
% \end{align*}
% It's easy to see that choosing $\eta = \sqrt{\nfrac{3}{\alpha\abs{S}}}\logv{\nfrac{2}{\delta}}$ yields
% \begin{align*}
%     \prvv{\abs{S'} \subset_{\alpha} \abs{S}}{\abs{S'} \in \insquare{1\pm\eta}\alpha\abs{S}} \ge 1-\delta
% \end{align*}
% and therefore $\nfrac{\abs{S'}}{\abs{S}} \in \alpha\insquare{1\pm\eta}$ with probability $1-\delta$. Taking a union bound, with probability $1-2\delta$, the number of bits to represent $k$ is at most
% \begin{align*}
%     &\ \log\logv{\nfrac{1}{\delta}}+\abs{S'}\logv{\frac{1}{\alphahat}} + \inparen{\abs{S}-\abs{S'}}\logv{\frac{1}{1-\alphahat}} \\
%     &= \log\logv{\nfrac{1}{\delta}}+\abs{S}\inparen{\frac{\abs{S'}}{\abs{S}}\logv{\frac{1}{\alphahat}} + \inparen{1-\frac{\abs{S'}}{\abs{S}}}\logv{\frac{1}{1-\alphahat}}} \\
%     &\le \log\logv{\nfrac{1}{\delta}}+\abs{S}\inparen{(1+\eta)\alpha\logv{\frac{1}{\alphahat}} + \inparen{1-(1-\eta)\alpha}\logv{\frac{1}{1-\alphahat}}} \\
%     &= \log\logv{\nfrac{1}{\delta}}+\abs{S}\inparen{\alpha\logv{\frac{1}{\alphahat}} + (1-\alpha)\logv{\frac{1}{1-\alphahat}} + \eta\alpha\logv{\frac{1}{\alphahat}}+\eta\alpha\logv{\frac{1}{1-\alphahat}}} \\
%     &= \log\logv{\nfrac{1}{\delta}}+\abs{S}\inparen{\kld{\alpha}{\alphahat} + H(\alpha) + \eta\alpha\logv{\frac{1}{\alphahat}}+\eta\alpha\logv{\frac{1}{1-\alphahat}}} \\
%     &\le \log\logv{\nfrac{1}{\delta}}+\abs{S}\inparen{\kld{\alpha}{\alphahat} + H(\alpha) + \eta\cdot\frac{\alpha}{\alphahat}}
% \end{align*}
% where the last line follows since $\alpha < \nfrac{1}{2}$ and $-x\inparen{\logv{x}+\logv{(1-x)}} < \nfrac{1}{2}$. We substitute our value of $\eta$ and conclude the proof of Lemma \ref{lemma:k_small}.
% \end{proof}
% We now choose a value of $\alphahat \ge \alpha$ that takes $o(n)$ bits to store while allowing us to bound $\kld{\alpha}{\alphahat}$.
% \begin{lemma}
% \label{lemma:choosing_alphahat}
% \nnote{choose $\alphahat$}
% \end{lemma}
% \begin{proof}[Proof of Lemma \ref{lemma:choosing_alphahat}]
% By Fact \ref{fact:pinsker}, we have
% \begin{align*}
%     \kld{\alpha}{\alphahat} \le \nfrac{1}{\alphahat} \cdot \inparen{\alpha-\alphahat}^2
% \end{align*}
% Let $\alphahat$ be the closest multiple of $\nfrac{1}{m}$ larger than 
% This concludes the proof of Lemma \ref{lemma:choosing_alphahat}.
% \end{proof}

% This concludes the proof of the upper bound of Theorem \ref{thm:short_hash_table_existence}.
% \end{proof}

% \begin{proof}[Lower bound, Theorem \ref{thm:short_hash_table_existence}]
% We reduce from a source coding task and apply the converse of Shannon's source coding theorem.

% \greenbox{
% \begin{center}
%     \underline{Source Coding Task}
% \end{center}
% The following task occurs between two parties (an \textit{encoder} and a \textit{decoder}).
% \begin{enumerate}
%     \item The universe samples $n$ objects independently at random according to $\cD^n$. Call this set $S_x$.
%     \item The universe tells the encoder and decoder $S_x$.
%     \item The universe chooses $S_y$ such that every element of $y$ is independently $\ber{\alpha}$.
%     \item The universe tells the encoder $S_y$.
%     \item The encoder sends a message $\cA$ to the decoder such that for every pair $(x,y) \in (S_x,S_y)$, the decoder can determine the value of $y$.
% \end{enumerate}
% }

% It is easy to see that the encoder and decoder can solve the task by writing and transmitting a program $\cA$ satisfying the requirements of Problem \ref{problem:short_hash_table}.

% Note that, assuming that $\cA$ indeed satisfies the requirements of Problem \ref{problem:short_hash_table}, we have for all $(x,y) \in S$ that $\cA(x) = y$. Thus, evaluating $\cA$ on every element in $S$ will tell the decoder the labels of every element of $S$. Finally, notice that this is exactly enough information to uniquely decode the original string $s$.

% By Shannon's source coding theorem, the expected length of $\cA$ must be at least $n \cdot H(\alpha)$. This is enough to conclude.
% \end{proof}


